Reasoning About a Service-oriented Programming Paradigm

This paper is about a new way for programming distributed applications: the service-oriented one. It is a concept paper based upon our experience in developing a theory and a language for programming services. Both the theoretical formalization and the language interpreter showed us the evidence that a new programming paradigm exists. In this paper we illustrate the basic features it is characterized by.

==> deployer.tex <==
\subsection{Deployment}
The deployment phase is in charge to bind service interface with network locations and protocols. A service, for example, could receive messages by exploiting the Http protocol or the SOAP over Http one, but the transport protocol choice is potentially unlimited. Such a task is achieved by means of port declarations. There are two kind of ports: \emph{input ports} and \emph{output ports}. The former ports allows for the declaration of all the input endpoints able to receive messages exhibited by the service engine, whereas the latter ones bind target location and transport protocol to the \emph{receiving services} of the behaviour. In other words the output port allows for the concrete connection with the services to invoke. In general we define a port as it follows:
\begin{quote}
\emph{A port is an endpoint equipped with a network address and a communication protocol joined to an interface whose operations will become able to receive or send requests. Ports which enables operations to receive requests are called input operations, output operations otherwise.}
\end{quote}
When deployed the service engine, if executed, is able to receive and send messages.



==> description.tex <==
\subsection{Service description}
A service description provides all the necessary information for interacting with a service. Service descriptions are composed by two parts: interface and deployment description.

\subsubsection{Interface.}
Service interfaces contain abstract information for performing compatibility checks between services. We identify three different levels of service interface:
\begin{itemize}
\item \textbf{Functional.} It reports all the input operations used by the behaviour for receiving messages from other services or applications. An operation description is characterized by a name, and its request and response message types. If we trace a comparison with the Web Service technology, such an interface level is well represented by the WSDL 1.1. specifications \cite{}.
At this level, only types checks on the interface are required in order to interact with the service.
\item \textbf{Work-flow.} It describes the work-flow of the behaviour. In a work-flow, input operations could not be always available to be invoked but they could be enabled by other message exchanges by implementing a sort of application protocol. Thus it is fundamental to know how a service work-flow behave in order to interact with it correctly. In the Web Service technology such an interface could be provided by means of an Abstract-BPEL~\cite{abstract-bpel} description but it is worth noting that also WSDL 2.0 specifications \cite{} now provide Message Exchange Patterns (MEP) which allows for the description of custom service interaction pattern. METTERE NELLE CONCLUSIONI CHE VOGLIAMO INTRODURRE QUESTO LIVELLO ANCHE IN JOLIE. At this level, also other approaches as the choreography one must be considered. Choreography languages, such as WS-CDL \cite{}, allows for the designing of the system from a global view point. In this case, a choreography can be exploited for describing the work-flow behaviour of a service by highlighting its role into the choreography. Thisis a wide area of investigation which involve works on contracts \cite{} and conformance \cite{} but it is not properly the focus of this paper. The reader interested in this topic may also consult \cite{other citations} \cite{contratti-wscdl-da-gigio}~\cite{gigio-contratti}~\cite{cmc-gnesi}.
\item \textbf{Semantics.} It offers semantic information about the service and the specific functionalities provided by it. It is provided by usually using some kind of onthology QUALCHE CITAZIONE FORSE ANCHE DAL WEB SEMANTICO E WEB 2.0. 
\end{itemize}

Service interfaces are strictly related to service discovery which is a key element of the service oriented programming paradigm. Nevertheless, discovery issues are properly related to search and compatibility algorithms over interfaces repositories also called \emph{registries}. These algorithms differ depending on which interface type is considered. 
It is out of the scope of this paper to discuss the different methodologies used for implementing service discovery. Here we want to highlight the fact that, at the present, some information related to service engine do not appear on the current interface standard proposals such as the sequential execution modality or the correlation set. These information are important to be specified into the interface because they could influence the system to build.


% Interesting results w.r.t. these topic have been achieved in~\cite{-



==> engine.tex <==
\subsection{Engine}
Here we present the concept of \emph{engine} we introduced in SOCK for dealing with those aspects of the service oriented programming paradigm related to the actual implementation of a service into a network. At the best of our knowledge does not exist a clear and precise definition of engine as we presented in SOCK. The motivations of such a lack could be probably found in the fact that it is a shared idea that the engine provides only the technologic support for implementing services without adding nothing fundamental. As far ad service oriented computing is concerned, engines are generally associated to those which execute WS-BPEL such as, for example, ActiveOS \cite{} or the Oracle one \cite{} but what about simple Web Services developed in Java, Python or .NET? Could we consider usual web servers such as IIS \cite{}, Apache \cite{}, JBoss \cite{} or Zope \cite{} as service engines? Do exist some characteristics on these applications which could be considered as basic features of the service oriented programming paradigm? In our perception the answer is yes and this section is devoted to highlight the main features a service engine is characterized by. In general we say that an engine is a machinery able to create, execute and manage service sessions. A more detailed definition of engine will be provided at the end of this section, now let us introduce the concept of session.
\subsubsection{Session.}
The definition of session follows:
\begin{quote}
\emph{A service session is an executing instance of a behaviour able to actually manipulate data.}
\end{quote}
We distinguish three different kinds of data resources, we call \emph{states}, which we can be accessed and modified by a session:
\begin{itemize}
\item a \textbf{local state} which is private and not visible to other sessions. We define such a kind of state a \emph{not persistent} state because it is deleted when the session finishes.
\item a \textbf{global state} which is shared among all the running sessions. We define suck a kind of state a \emph{persistent} state because it is deleted only when the engine is stopped.
\item a \textbf{storage state} which is persistent and shared among all the running sessions whose persistence is independent from the execution of a service engine (e.g. a database).
\end{itemize}
A key element of the service oriented programming paradigm is session identification. In general a session is identified by its own local state or a subpart of it. The subpart of the local state which identifies a session can be programmed and it is called \emph{correlation set}. Corralion set is a mechanism provided by WS-BPEL and it has been formalized in SOCK, COWS \cite{} and in \cite{viroli citazione}. Also in JOLIE we chose to allow for the correlation set specification. In order to explain better such a mechanism let us introduce a simple notation where a session is represented by a couple of terms $(P,S)$ where $P$ represents a behaviour in a given formalism and $S$ represents the local state here modelled as a function from variables to names. ${\mathcal S}: Var\rightarrow Names$ where $Var$ is the set of variables and $Names$ the set of names. Now, let us consider two sessions with same behaviour but different local states $S_1$ and $S_2$:
$$s_1:=(P,S_1)\ \ s_2:=(P,S_2)$$
We say that $s_1$ is not distinguishable from $s_2$ if $S_1=S_2$\footnote{Let ${\mathcal S}$ be the set of states, we define $=:({\mathcal S}\times {\mathcal S})$ where $S_1 = S_2$ if $S_1(x)=S_2(x)$ and $Dom(S_1)=Dom(S_2)$}. Now, let us consider both ${\mathcal S_1}$ and ${\mathcal S_2}$ as a composition of states defined on disjoint domains:
$${\mathcal S_1}=S_{11}\oplus S_{12}\oplus S_{13}\ \ ,\ Dom(S_{11})\cap Dom(S_{12}) \cap Dom(S_{13}) = \emptyset $$
$${\mathcal S_2}=S_{21}\oplus S_{22}\oplus S_{23}\ \ ,\ Dom(S_{21})\cap Dom(S_{22}) \cap Dom(S_{23}) = \emptyset $$
where the operator $\oplus$ represents a composition operator over states\footnote{$\oplus:{\mathcal S}\times {\mathcal S}\rightarrow {\mathcal S}$ where $S_1\oplus S_2(x) = S_1(x)\ if x\in Dom(S_1), S_2(x)\ if\ x\in Dom(S_2)\cap x\notin Dom(S_2), undefined\ otherwise$}. Let us consider $S_{11}$ and $S_{21}$ as the correlation sets for $s_1$ and $s_2$ respectively. We say that $s_1$ is not distinguishable from $s_2$ if $S_{11}=S_{21}$.

It is worth noting that such a session identification mechanism for the service oriented programming paradigm differs from that of the object oriented one. In the object oriented approach indeed, an object is always identified by the reference issued at the moment of the object creation. 

\subsubsection{Session management.}
The main activity of a service engine is the session management. In order to achieve this task it provides the following functionalities:
\begin{itemize}
\item \textbf{Session creation}. Sessions can be created in two different ways:
\begin{itemize}
\item when an external message is received on a particular operation of the behaviour. Some operations can be marked as session initiators. When a message is received on a session initiator operation, a session can be started.
\item when a user manually starts it. A user can launch a service engine which immediately executes a session without waiting for an external message. We usually denote such a session as a \emph{firing session}.
\end{itemize}
\item \textbf{State support}. When a session is created, a private state is immediately joined to it. The service engine also provides the support for the global state which is shared among all the sessions. Moreover, it provides the connectors for interacting with the storage states.
\item \textbf{Message routing.} Since a session is identified by its correlation set, the engine must provide the mechanisms for routing the incoming messages to the right session. The session identification issue indeed, is raised every time a message is received. For the sake of generality, in a service oriented programming paradigm, we cannot assume that some underlying application protocols such as WS-Addressing \cite{ws-Addr} or other transport protocol identification mechanisms such as Http Cookies \cite{} are always used for identifying sessions; here is why Web Services are considered \emph{loosely coupled}. We consider the correlation set as the representative mechanism for routing incoming messages in the service oriented programming pardigm. Its functioning can be summarized as it follows. Thus it can be seen as a function from variables to names: $m\in{\mathcal S}$. As we have done for the states we can define a correlation set also for a message. Now, we define the correlation function $c:Var\rightarrow Var$ and we say that a message $m$ must be routed to the session $s$ if:
$$\forall x\in Dom(M_1) \Rightarrow s(c(x)) = m(x) \vee s(c(x))\ is\ udenfined\ \wedge c(x)\in S_1$$ 
where $M_1$ and $S_1$ are the correlation sets for $m$ and $s$ respectively. In other words, a message can be routed to a session only if its correlated data correspond to those of the session.

\item \textbf{Session execution}. Sessions can be executed sequentally or concurrently. It is a shared idea that sessions are executed concurrently but the sequential case allows for the controlling of some specific hardware resources which need to be accessed sequentially. As an example let us consider a withdrawal machine which starts sessions sequentially due to its harware nature. It can be argued that sequentiality could be modelled by exploiting concurrent execution with synchronizations over the global state and it does not deserve to be considered as a key aspect of the service oriented programming paradigm, but we consider such an aspect fundamental from an architectural view point because it can raise system deadlock issues if not considered, as we have shown in \cite{} by means of SOCK.
\end{itemize}


\subsubsection{Engine definition.}
Now, we can provide our definition for the service engine:
\begin{quote}
\emph{An engine is a machinery able to manage service sessions by providing session creation, state support, message routing and session execution capabilities.}
\end{quote}



==> eptcsdata.tex <==
\providecommand{\event}{M.H. ter Beek (Ed.): Young Researchers Workshop\\
on Service-Oriented Computing 2009 (YR-SOC'09).
}
\providecommand{\volume}{2}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{67}
\providecommand{\eid}{6}

